Conversation Style Transfer using Few-Shot Learning

Conventional text style transfer approaches focus on sentence-level style transfer without considering contextual information, and the style is described with attributes (e.g., formality). When applying style transfer in conversations such as task-oriented dialogues, existing approaches suffer from these limitations as context can play an important role and the style attributes are often difficult to define in conversations. In this paper, we introduce conversation style transfer as a few-shot learning problem, where the model learns to perform style transfer by observing only a few example dialogues in the target style. We propose a novel in-context learning approach to solve the task with style-free dialogues as a pivot. Human evaluation shows that by incorporating multi-turn context, the model is able to match the target style while having better appropriateness and semantic correctness compared to utterance/sentence-level style transfer. Additionally, we show that conversation style transfer can also benefit downstream tasks. For example, in multi-domain intent classification tasks, the F1 scores improve after transferring the style of training data to match the style of the test data.

==> 1introduction_old.tex <==
\section{Introduction}\label{sec:introduction}
With the recent advances in neural dialogue models \citep{gao2018neural,zhang2020recent,ni2022recent}, the conversational agents are capable of solving increasingly complex tasks. However, one key challenge for adopting these agents is achieving desired conversational style. Even when providing similar functionality, the requirement of conversational style is often different depending on the domain and use case (e.g., banking vs restaurant agents) or the user profile (e.g., conversation with senior people vs youngsters).
% \nikos{Can we give an example to make it easier to grasp?}
%Such style requirement might also change dynamically based on the user profile (e.g., senior people vs youngsters). 

Style transfer in NLP has been studied as the problem of transferring the text from one known style to another \citep{pavlick2016empirical,rao2018dear,niu2018multi,wang2019harnessing,briakou2021ola}. Existing methods for style transfer operate at the sentence level and ignore the inter-sentential context. However, in conversational domains such as task-oriented dialogues (TODs), the context plays an important role and performing style transfer at the sentence-level can result in an inappropriate response as demonstrated in Figure \ref{fig:problem-formulation}.

%With the recent advance in neural dialogue models \citep{gao2018neural,zhang2020recent,ni2022recent}, the conversational agents are capable of solving increasingly complex tasks. However, one key challenge for adopting these agents is to achieve desired conversational style. The challenges in a conversational style are often different as it depends on the domain and use case (e.g., banking vs restaurant agents). The conversation style requirements might also change dynamically within a conversation based on the user profile (e.g., senior people vs youngsters) or situation (e.g., talking to someone angry vs someone depressed).

%In this paper, we define the novel problem of conversation style transfer by addressing some key challenges in this task. Firstly, style transfer in NLP has been studied as the problem of transferring the text from one known style to another \citep{pavlick2016empirical,rao2018dear,niu2018multi,wang2019harnessing,briakou2021ola} and the existing methods for style transfer operate at the sentence level ignoring the inter-sentential context. However, in conversational domains such as task-oriented dialogues (TODs), the context plays an important role, and performing style transfer at the sentence level can result in an inappropriate response as demonstrated in Figure \ref{fig:problem-formulation}.

% \nikos{Can we give an example to make it easier to grasp?}
%Such style requirement might also change dynamically based on the user profile (e.g., senior people vs youngsters). 

\begin{figure}[t!]
  \includegraphics[width=0.47\textwidth]{figures/intro-example-v4.pdf}
  \caption{Transferring the style of an utterance from chatbot to human agent style based on three utterance-level (single-turn) and conversation-level (multi-turn) examples as input. Additional conversational context helps the style transfer model to yield a more appropriate response as the dialogue contains useful information that can be leveraged during the generation process. 
  
  %\sm{small font, can increase?}
  %\nikos{several points:  i) this diagram could be simplified but not sure how; one idea would be to show only the conversational level style transfer part and highlight with gray what is given as context to the utterance-level model along with the two different responses. ii) the "training" part is a bit confusing since the proposed method uses only in-context learning. can't we simply show directly the "prompt" and the generated response?  iii) adding an explanation of why that is would help e.g. by taking into account conversational context}
  }
  \label{fig:problem-formulation}
\end{figure}

The existing approaches for style transfer assume that the style attributes are known and well defined (e.g., politeness and friendliness) \citep{zhang2018style,madaan2020politeness,reif2022recipe}. However, defining the style of a conversation with such attributes is challenging and due to the dynamic nature of conversations, the conversation style may be a combination of many style attributes. Examples from TWCS dataset~\cite{stuart_axelbrooke_2017} in Table \ref{tab:off-the-shelf-example} show that the agent responses from Chipotle and VirginTrains services are classified to have similar politeness scores by an off-the-shelf politeness classifier \cite{danescu2013computational} but their actual styles are drastically different upon a closer look. Chipotle responses are conversational and friendly and VirginTrains responses are direct. 
%\nikos{What are the differences? I suggest to mention them explicitly and  point to a specific cell in the table.}

%\begin{figure}[t!]
%  \includegraphics[width=0.48\textwidth]{figures/examples-style-attributes.pdf}
%  \caption{Limitation\sm{the limitation is not clear, can add a sentence explaining? also need to increase font} of defining style using fixed attributes (Politeness). The conversations from different companies are taken from Customer Support in Twitter (TWCS) dataset \cite{danescu2013computational}. The politeness score is calculated using Stanford Politeness API \cite{danescu2013computational} \shu{change company names to Company1, Company2}. 
%  }
%  \label{fig:off-the-shelf-example}
%\end{figure}

\begin{table}
\centering
\resizebox{1\columnwidth}{!}{%
\begin{tabular}
{>{\arraybackslash}m{8.3cm}>{\centering\arraybackslash}m{2cm}>{\centering\arraybackslash}m{2.3cm}}

\toprule
\textbf{\makecell[c]{Example \\ conversations }} & \textbf{Avg. politeness} & \textbf{Intuitive style attributes}\\
\midrule
%\textbf{\rotatebox[origin=c]{90}{Chipotle}} & 
\makecell[l]{\textsc{\textbf{\underline{Chipotle}}}\\\textbf{[Customer]} \$3 burritos and I’m nowhere near a Chipotle\\\textbf{[Agent]} Bummer. I'm so sorry. How far away is the clos-\\est location? –Becky} & 0.51 & \makecell[l]{Friendly,\\Conversational,\\Not-Impolite}\\
\midrule

 %\textbf{\rotatebox[origin=c]{90}{Comcast}} & 
 \makecell[l]{\textsc{\textbf{\underline{Comcast}}}\\\textbf{[Customer]} My internet is down and xfinity talkin about\\24-72 hours... y’all have the game messed up.\\\textbf{[Agent]} I understand this is a frustrating experience,\\please send a DM with your account information so I can\\look into this matter for you} & 0.77 & \makecell[l]{Formal,\\Task-Oriented}\\
\midrule

 %\textbf{\rotatebox[origin=c]{90}{\makecell[c]{Virgin-\\Trains}}} & 
 \makecell[l]{\textsc{\textbf{\underline{VirginTrains}}}\\\textbf{[Customer]} See attached error message. I've tried leaving\\a voicemail several times in the past week.\\\textbf{[Agent]} Have you tried from another device?} & 0.50 & \makecell[l]{Direct,\\To-the-point,\\Bot-like}\\


\bottomrule
\end{tabular}}
%\caption{\nikos{Columns could be simply "Examples", "Avg. Politeness" or "Avg P.", "Style" and company name could be added in a row just above the data row to save some horizontal space and hopefully increase font size.}Limitation\sm{the limitation is not clear, can add a sentence explaining? also need to increase font} of defining style using fixed attributes (Politeness). The conversations from different companies are taken from Customer Support in Twitter (TWCS) dataset \cite{stuart_axelbrooke_2017}. The politeness score is calculated using Stanford Politeness API \cite{danescu2013computational} \shu{change company names to Company1, Company2}.}
  
  \caption{Example conversations of customer care agents from TWCS dataset that show the limitation of style definitions using fixed attributes, here politeness. Chipotle and VirginTrains customer care agents get roughly the same politeness score by an off-the-shelf politeness classifier \cite{danescu2013computational} though intuitively their style attributes are different. 
  %as shown in the third column. %\nikos{move 3rd column all the way to the left?}
  }
  \label{tab:off-the-shelf-example}
\end{table}



%\begin{table}
%\centering
%\resizebox{1\columnwidth}{!}{%
%\begin{tabular}
%{>{\arraybackslash}m{2.3cm}>{\centering\arraybackslash}m{1.8cm}>{\centering\arraybackslash}m{8.3cm}}
%
%\toprule
%\textbf{Intuitive Style att.} & \textbf{Avg. politeness} & \textbf{\makecell[c]{Example \\ conversations }} \\
%\midrule
%\textbf{\textsc{Chipotle}} & &\\
%\midrule
%\textbf{\rotatebox[origin=c]{90}{Chipotle}} & 
% \makecell[l]{{\textsc{Chipotle}} \vspace{1mm} \\ Friendly,\\Conversational,\\Not-Impolite} & 0.51 & \makecell[l]{ \textbf{[Customer]} \$3 burritos and I’m nowhere near a Chipotle\\\textbf{[Agent]} Bummer. I'm so sorry. How far away is the clos-\\est location? –Becky} \\
%\midrule
%
 %\textbf{\rotatebox[origin=c]{90}{Comcast}} & 
% \makecell[l]{\textsc{Comcast} \vspace{1mm} \\ Formal,\\Task-Oriented} & 0.77 & \makecell[l]{\textbf{[Customer]} My internet is down and xfinity talkin about\\24-72 hours... y’all have the game messed up.\\\textbf{[Agent]} I understand this is a frustrating experience,\\please send a DM with your account information so I can\\look into this matter for you}\\
%\midrule
%
 %\textbf{\rotatebox[origin=c]{90}{\makecell[c]{Virgin-\\Trains}}} & 
% \makecell[l]{\textsc{VirginTrains} \vspace{1mm} \\ Direct,\\To-the-point,\\Bot-like} & 0.50 & \makecell[l]{\textbf{[Customer]} See attached error message. I've tried leaving\\a voicemail several times in the past week.\\\textbf{[Agent]} Have you tried from another device?}\\


%\bottomrule
%\end{tabular}}
%  \caption{Example conversations of customer care agents from TWCS dataset that show the limitation of style definitions using fixed attributes, here Politeness. Chipotle and VirginTrains customer care agents get roughly the same politeness score by an off-the-shelf politeness classifier \cite{danescu2013computational} though intuitively their style attributes are different as shown in the third column. \nikos{move 3rd column all the way to the left?}}
%  \label{tab:off-the-shelf-example}
%\end{table}




In this paper, we define a new task 
%\nikos{why not simply "task"}
of \textit{conversation style transfer} by using only a few example dialogues in the target style. In this setting, we do not need to interpret the style attributes of the source/target dialogues. Also, we do not require parallel data in the form source-to-target pairs, which is expensive and difficult to collect. We show that such a task design can benefit several applications such as chatbot personalization and data augmentation in down-stream tasks.
%\nikos{If there are any annotations that proposed method requires beyond the few examples, this is the right place to mention. } 

To address the few-shot learning problem, we propose a novel method based on in-context learning~\cite{brown2020language}. We propose to perform source-to-target style transfer with a style-free dialogue as pivot. In this approach, we first prompt pre-trained large language models (LLMs) to perform style reduction on source dialogue, then use another set of prompts to rewrite the style-free dialogue to match the target style. To accurately and efficiently evaluate the quality of conversational style transfer with different models, we conduct a ranking-based human assessment on style strength, appropriateness and semantic correctness. The appropriateness assessment is unique to conversation style transfer, which evaluates whether the transferred utterances are out-of-context. As supplementary metrics, we report automatic scores including classifier-based style strength and semantic similarity scores.
We observe that utterance-level style transfer without contextual information can achieve the highest style strength scores, however, results in low appropriateness and semantic correctness. On the other hand, by including contextual information %, although with lower style strength,
the transferred utterances are more appropriate and semantically correct.




%\nikos{these last two paragraphs can be merged.}
%\nikos{how do we obtain the style free dialogue annotations and how expensive they are to obtain? mention explicitly.}. 
\removedbyraph{
As as first step, we construct pseudo parallel data containing source-style dialogues and style-free dialogues. %\nikos{how are these pseudo parallel data constructed exactly?}.
We use these examples to prompt the LLMs to perform automatic style reduction on source-style dialogues to obtain the style-free version. In the second step, we construct pseudo parallel data in a similar way, then prompt the language models to transfer the style-free dialogues into the target style. In this approach, we use human supervision to construct parallel examples for styled to style-free dialogues only, which is easier to achieve as it does not require humans to have domain knowledge about the target style.
}
%\sm{can be shortened as might be repetitive with approach section}


% In conversational style transfer, it is essential that change in style does not cause the sentence to be out-of-context. For chatbot personalization, we perform automatic and human evaluation of style strength, appropriateness and semantic correctness. Our key finding is that utterance-level style transfer with no context achieves high style strength scores, however, results in more inappropriate and semantically incorrect responses from the chatbot. On the other hand, by including contextual information, lower style strength is observed but the responses are more appropriate and semantically correct. \nikos{Can we say something about the effect of model size?}

%The evaluation is mainly done through ranking-based human evaluation. Additionally, we also propose automatic metrics as supportive metrics. We compare the conversational style transfer models with different context window: no context, short segment, long segment. We found that utterance-level style transfer with no context achieves high style strength scores, however, results in more inappropriate and semantically incorrect responses from the chatbot. On the other hand, by including contextual information, lower style strength is observed but the responses are more appropriate and semantically correct. 

To evaluate the impact of conversational style transfer for data augmentation, we perform extrinsic evaluation by transferring the style of training data for intent classification task. We experiment in the setting where the training and test data are having different styles. We apply few-shot conversation style transfer on the training data to convert it to the test style before training. As a result, we observe
%1.06\%, 1.15\% and 0.46\% 
improvement on intent classification F1 scores across three domains. The results demonstrate the usefulness of style transfer of conversations in down-stream applications.
%in Insurance, Banking and Finance customer care domains, respectively.\sm{you can shorten or remove the last paragraphs and keep results to abstract, summary and results section, a good suggestion bu Nikos is to include a summary of novelty/contributions and perhaps the paper structure}

%\nikos{A summary of the key contributions in a few short bullet points provides a quick reference/recap that can help readers more easily remember them.}
% \nikos{last four paragraphs can be simplified; let's make it more concise.}

==> 4data.tex <==
\section{Data Collection}\label{sec:data-collection}


==> 7evaluation.tex <==
\begin{figure*}[h!]
  \includegraphics[width=1\textwidth]{figures/evaluation-metrics.pdf}
  \caption{Examples of style transfer evaluation metrics: \textit{style strength, appropriateness and semantic correctness.} }%\nikos{nice!!}
  \label{fig:evaluation-metrics}
\end{figure*}

\section{Evaluation Techniques}\label{sec:evaluation}
In this section we describe the evaluation techniques for our models performance for style transfer in Task Oriented Dialogues (TODs). We limit our study to style transfer of one speaker of a conversation in two speakers TODs, that are customer care agents.
%\footnote{We leave the study on the style of the customers as a future work because different customers may have different style and it is practically impossible to have a control over that.}

\subsection{Evaluation Metrics}
%We evaluate our models performance in the following three aspects.
\nikos{use bullet points?}
\noindent\textbf{Style Strength:} Following previous studies \citep{reif2022recipe,han-etal-2022-meet} we evaluate the target style strength in a style transferred utterance. It can be defined as how similar in style is the style transferred utterance to the target style. %\nikos{How is the similarity defined exactly?}
    
\noindent\textbf{Semantic Correctness:} Semantic correctness in the context of TODs can be defined as the preservation of intents in the style transferred utterances. In TODs we need to preserve the intents in the source utterances in the style transferred version of them to prevent bad customer experience. %So we evaluate how well the models can preserve the semantic meaning after style transfer. \nikos{Definition?}
    
\noindent\textbf{Appropriateness of Response:} Appropriateness of response in TODs can be defined as the appropriateness of an agent's response given the previous customer turn in a conversation. This is especially required in TODs for better customer experience. 

Some positive and negative examples of these metrics can be found in Figure \ref{fig:evaluation-metrics}.

%We evaluate the appropriateness of agent responses after style transfer. This is especially required in TODs. We evaluate if the model generates any awkward response in order to transfer an utterance to a target style. Consider a scenario when a customer says, \textit{"I had an accident and I want to file an auto insurance claim"}. An agent's response in this scenario in a style that is direct can be, \textit{"What is your insurance number?"}. To transfer the style to more conversational and formal if the model transfers it to - \textit{"I am happy to hear that. Can I get your insurance number?"}, it will be an inappropriate response given the context. An appropriate style transferred response in this scenario would be \textit{"I am sorry to hear that. Can I get your insurance number?"}. \nikos{same. see comments above.}



\subsection{Automatic Evaluation}
To measure the strength of the target style automatically we train a RoBERTa \cite{liu2019roberta} based binary text classifier to classify between the source style and the target style.%\nikos{This seems to be following previous practice. Can we point to relevant papers?}
We pre-train this classifier to classify between the source and the target style using the additional dataset from corresponding corpus. We run this classifier on source conversations and the corresponding style transferred conversations and use this classifiers confidence on the target style as the target style strength score. 

%\nikos{this would better fit in the section above} 
We measure the semantic similarity between the source utterances and the corresponding style transferred utterances by taking the cosine similarity between the source and the style transferred utterances in the semantic meaning-based representation space as described in Section \ref{subsection:dynamic-prompt-selection}. 

To the best of our knowledge it is difficult to get an automatic method to measure the appropriateness of response and so we rely \textbf{only} on human evaluation for this. %\nikos{This is a bit confusing. Does it mean that semantic similarity is always calculated in an automatic way? Please specify. Can we have a high-level view of the different characteristics and how they are defined (human vs automatic vs both? }

Note that, judgment of style can be very subjective and so automatic evaluation techniques for measuring the style strength only can provide us with an approximation of the quality of the target style. Moreover, getting additional dataset in target style to train a style classifier may not be possible in real life scenarios. When evaluating semantic correctness two utterances may get a high semantic similarity score and still may not preserve the meaning totally. So, we additionally perform human evaluation for all of the three criteria described above. \nikos{The final two paragraphs can be merged. The main message is that automatic metrics are not very reliable and we need to resort to human evaluation.}


\subsection{Human Evaluation} To perform human evaluation for style strength and appropriateness of response, we rely on ranking based human evaluation among our proposed models and the baseline. To evaluate style strength, we present human evaluators with some utterances in the target style domain to learn about the style properties of the target style. Then we present them with a source utterance and the style transferred versions of it by our proposed models and the baseline. Note that the model names were kept hidden from the human evaluators and the order of the utterances were randomly shuffled for each data point. Then we asked the human evaluators to rank all of the versions of the same utterance in a descending order based on the style similarity with the reference utterances. \nikos{ how did we aggregate the rankings from the different annotators?} We follow the same ranking based approach for evaluating appropriateness of response. We present human evaluators with all versions of the style transferred agent utterances of the same agent utterance along with the immediate previous customer turn as context and ask the human annotators to rank them based on the appropriateness of the agent response. %\nikos{What were the exact instructions to the annotators? This is a good place to add a reference to it in the supplementary material.}

For evaluation of semantic correctness we present human evaluators with a source utterance and the corresponding style transferred utterances by the models. Then we ask them for each style transferred version if it is semantically similar, partially similar or dissimilar to the source utterance.

Each data point was evaluated by three human evaluators and we didn't include data points where all of the models generated exactly the same response. \nikos{which platform did we use for the annotation?} Details on the human evaluation dataset statistics, evaluation interfaces, and inter-annotator agreement measures can be found in Appendix \ref{appendix:human-evaluation}.



%\subsection{Human Evaluation} The human evaluation techniques for all of the three metrics are described below.

%\begin{itemize}
%    \item \textbf{Style Strength} We present human evaluators with some reference utterances in the target style. Then we present them with style transferred utterances of the same source utterance by two versions of our model (2-turn and 4/5-turn conversations) and the baseline (utterance level). In addition to that we present them the source utterance itself. Then we ask the human annotators to rank the 4 versions of the same utterance in a descending order based on the style similarity with the reference utterances. The model names were hidden from the annotators and the four versions were presented in a randomly shuffled order for each example. Note that, when doing style transfer at 4/5-turn conversation level, it may result in non-parallel conversation compared to the source conversation because of turn reduction by the model. To match the non-parallel utterances with the source utterances, we rank the style transferred utterances based on their semantic similarity with the source utterances and pick the one with the highest similarity. We discard any style transferred utterance that has the highest semantic similarity of less than 0.2.  
%    \item \textbf{Appropriateness} We present human evaluators with 4 versions of the agent turns of the same agent utterance as described above along with the immediate previous customer turn as context and ask the human annotators to rank them based on the appropriateness of the agent response. The most appropriate response gets a rank of 1 and the least appropriate response gets a rank of 4.
%    \item \textbf{Semantic Correctness} We present the human evaluators with the source utterance and the corresponding style transferred utterances by the models (including baseline). Then we ask them for each style transferred utterance if it is semantically similar, partially similar or dissimilar to the source utterance.
%\end{itemize}






==> 8downstream_application.tex <==
\section{Downstream Application}\label{sec:downstream-application}
The downstream application of conversation style transfer is understudied. In this paper, we apply conversation style transfer in a downstream application of Intent Classification. We focus on the setting where we have abundant of training data in one style domain and the test data comes from a different style domain. We use the DST11 dataset where the training data are human-to-human conversations and the test data are human-to-bot conversations. We first convert the style of the training data to the style of test data using few shot examples from the test data, then use this style transferred data for training the intent classifier. The intent classification results improves when the style transferred data is used as training data. The results for three different domains of the DSTC11 dataset are shown in Table \ref{tab:ic-results-f1-score}. The detailed data collection process and statistics can be found in Appendix \ref{appendix:downstream-application}. %We run this experiment on the setting where few shot training is done for the intent classifier that are reported in Appendix \ref{appendix:downstream-application} along with the whole dataset statistics. We left other downstream applications of conversation style transfer as future work.  

\begin{table}[ht]
\centering
\resizebox{1\columnwidth}{!}{%
\begin{tabular}
{>{\arraybackslash}m{4cm}>{\centering\arraybackslash}m{1.9cm}>{\centering\arraybackslash}m{1.7cm}>{\centering\arraybackslash}m{1.8cm}}

\toprule
    \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{F1 score on test data (hum.-to-bot conv.)}}\\
    \cmidrule(lr){2-4}
    \textbf{Training data} & \textbf{Insurance (21 classes)} & \textbf{Banking (9 classes)} & \textbf{Finance (23 classes)}\\
    \cmidrule(lr){1-4}
    hum.-to-hum. conv. & 93.37 (1.0) & 94.95 (4.0) & 89.29 (0.5)\\
    hum.-to-hum. conv. transferred to hum.-to-bot style & \textbf{94.43 (1.4)} & \textbf{96.1 (3.2)} & \textbf{89.75 (0.3)}\\
    \bottomrule
\end{tabular}}
\caption{Intent classification results.}\label{tab:ic-results-f1-score}
\end{table}


%Conversation style transfer can be of many use including synthesizing training examples for downstream tasks such as Intent Classification, Slot Labeling, and so on. Downstream applications of style transfer are understudied. In this paper we take the first step towards one of the downstream applications of style transfer of TODs namely Intent Classification. Few-shot conversation style transfer can be of real use when we have abundant of training data from one style domain and the test data comes from a different style domain. We study the usefulness of style transfer in such setting for a downstream Intent Classification (IC) task. We have training data from human-to-human style domain and test data from human-to-bot style domain from DSTC11 dataset. We convert the style of the human-to-human conversations to human-to-bot before training the intent classification model and observe the effect of that in the test performance. Mostly the customer utterances are annotated for intents in this dataset. So, instead of converting the style of the agent utterances we convert the style of the customer utterances using our proposed model. As we require a large amount of data for this training and style transfer is an expensive operation, we use GPT-NeoX as a language model for this task. We use the utterance level style transfer as it shows the highest style strength among all of the versions for this task. 
